Axial-field-induced chiral channels in an acoustic Weyl system

Condensed-matter and other engineered systems, such as cold atoms, photonic, or phononic metamaterials, have proven to be versatile platforms for the observation of low-energy counterparts of elementary particles from relativistic field theories. These include the celebrated Majorana modes, as well as Dirac and Weyl fermions. An intriguing feature of the Weyl equation is the chiral symmetry, where the two chiral sectors have an independent gauge freedom. While this freedom leads to a quantum anomaly, there is no corresponding axial background field coupling differently to opposite chiralities in quantum electrodynamics. Here, we provide the experimental characterization of the effect of such an axial field in an acoustic metamaterial. We implement the axial field through an inhomogeneous potential and observe the induced chiral Landau levels. From the metamaterials perspective these chiral channels open the possibility for the observation of non-local Weyl orbits and might enable unidirectional bulk transport in a time-reversal invariant system.

==> fig1caption.tex <==
%!TEX root=manuscript.tex
\caption{
%
{\bf Inhomogeneous Weyl point separation and axial magnetic fields.} {\bf a,} Hexagonal Brillouin zone with the high-symmetry points $\Gamma$,$K$,$K'$,$H$, and $H'$. The blue (red) dots indicate schematically Weyl points of chirality $s=+1$ ($-1$) whose location in momentum space is shifted as a function of the spatial coordinate $x$ due to the presence of an axial magnetic field. {\bf b,} Tight binding model and the local acoustic orbitals in the structure shown in {\bf c}. The density plot indicates the pressure field in the mid-plane of the the cavity at $h/2$. The colors mark the phases of the local modes. {\bf c,} Unit-cell of the hexagonal acoustic crystal. The parameters are explained in the main text. {\bf d,} Chiral Landau levels emerging at the high-symmetry points due to the axial magnetic field. The color again indicates the chirality of the Weyl points. {\bf e,} Photo of the acoustic crystal.
%
} 

==> fig2caption.tex <==
%!TEX root=manuscript.tex
\caption{
%
{\bf Observation of chiral Landau levels.} {\bf a,} High-symmetry lines in the Brillouin zone and projection of the $x$-axis onto $k_y,k_z$. {\bf b,} Fourier transform to the first Brillouin zone at $k_z=0$ ($k_z=\pi/a_z$ shows similar behavior which is not shown.) of the acoustic response at different frequencies for different speaker positions (top, bottom, right, or left, see text). The concentration of the response at $7.7\,{\rm kHz}$ around the $K$ and $K'$ points shows that physics at these frequencies is governed by the band-touchings at the corners of the Brillouin zone. The excitation sensitivity of the $K$ and $K'$ at $7.7\,{\rm kHz}$ strongly indicates chiral channels, see text. At lower (higher) frequencies, the response is dominated by a spherically symmetric spectrum.  {\bf c,} Quantitative analysis of the above density plots for $7.7\,{\rm kHz}$ (solid lines) and $7.0\,{\rm kHz}$ (dashed lines), showing that at $7.0\,{\rm kHz}$ the response is already dominated by the $K$ and $K'$ points. At $7.7\,{\rm kHz}$, the chiral Landau levels lead to an imbalance between $K$ and $K'$ as a function of excitation location. {\bf d,} Measured spectrum along the high-symmetry lines indicated in {\bf a}. Both for the top and bottom panel one can observe the touching of two bands around $7.7\,{\rm kHz}$. Overlaid is the analysis presented in {\bf e}. The middle panel shows a gap opening along the $K$-$H$ lines. {\bf e,} Dispersion along the chiral Landau levels at the four high-symmetry points in the Brillouin zone. The momentum-frequency relation was obtained via fitting the phase evolution of the measured frequency response (see text). The horizontal error-bars, reflecting the error in fitting, are smaller than the symbol size. The vertical error bars indicate our frequency uncertainty given the dissipation in the acoustic field.
} 

==> fig3caption.tex <==
%!TEX root=manuscript.tex
\caption{
%
{\bf Characterisation of surface Fermi arcs.} {\bf a,} Surface Fourier-transform of the measured Fermi arc on the $+\hat {\bf x}$ surface. The white curved lines show the location of the maximal response. This is obtained fitting the response at fixed frequency and $k_z$ with a Lorentzian in order to find the $k_y$ with maximal response as shown in {\bf c} for $k_z$ marked with a dashed line. {\bf b,} Evolution of the white curved lines in {\bf a} as a function of frequency $\omega$ on the two surfaces $\pm \hat {\bf x}$ (top, bottom). The opposite sign of the group velocity $v_y=\partial_{k_y}\omega$ indicate the chiral nature of the surface modes winding around the sample according to the $k_z$-layer Chern number.
%
} 
